Strict lower bounds with separation of sources of error in non-overlapping domain decomposition methods

This article deals with the computation of guaranteed lower bounds of the error in the framework of finite element (FE) and domain decomposition (DD) methods. In addition to a fully parallel computation, the proposed lower bounds separate the algebraic error (due to the use of a DD iterative solver) from the discretization error (due to the FE), which enables the steering of the iterative solver by the discretization error. These lower bounds are also used to improve the goal-oriented error estimation in a substructured context. Assessments on 2D static linear mechanic problems illustrate the relevance of the separation of sources of error and the lower bounds' independence from the substructuring. We also steer the iterative solver by an objective of precision on a quantity of interest. This strategy consists in a sequence of solvings and takes advantage of adaptive remeshing and recycling of search directions.

==> Separation_of_algebraic_error_and_discretization_error.tex <==


Our objective is to separate the contributions to the global error of the discretization error and of the algebraic error, so that a new stopping criterion for the iterative solver can be defined, avoiding useless iterations that cannot reduce the global error (see Figure~\ref{fig:courbe_L}).\medskip



First, we exhibit a new bound which, compared to~\eqref{eq:estimgus}, involves   $\un{u}_N$ instead of $\un{u}_D$, this upper bound of $ \vvvert  \un{u}_{ex}-\un{u}_N  \vvvert _{\Omega} $  distinguishes the algebraic error due to the use of the DD iterative solver from the discretization error due to the finite element approximation.

The fundamental result is the following theorem:
\begin{thm}\label{thm:separation}
Using the notation of algorithms~\ref{alg:bdd} or~\ref{alg:feti}, we have
\begin{equation}
 \vvvert  \un{u}_{ex}-\un{u}_N  \vvvert _{\Omega} \leq  \sqrt{\res^T\bz} + \sqrt{\sum_s\ecrc{\dep_N\s,\hat{\sig}_N\s}{\Omega\s}}
\end{equation}
\end{thm}
In other words, at each iteration of the solver, the distance between the displacement field $\un{u}_N$ and the exact solution is bounded by the preconditioner norm of the residual of the conjugate gradient solver plus a sum over subdomains of errors in constitutive relation which depend on the iteration and on the discretization and which are computed in parallel.

The preconditioner-norm of the residual is a purely algebraic quantity computed during the conjugate gradient iterations,  it can be used in order to tell the convergence of the algorithm. In the assessments, we will verify that the term $\sqrt{\sum_s\ecrc{\dep_N\s,\hat{\sig}_N\s}{\Omega\s}}$ is mostly driven by the discretization, so that it varies slightly during the iterations.\medskip

The proof of the theorem is based on two lemmas.
\begin{lem}\label{thm:separation_continue}
Let $\un{u}_{ex}\in\KA(\Omega)$ solve the reference problem \eqref{eq:refpb}, $(\un{u}_D\s)_s\in\KA(\Omega)$ and $(\un{u}_N\s)_s\in\broken$ be as defined in Section~\ref{ssec:apee}, then:
\begin{equation}
 \vvvert  \un{u}_{ex}-\un{u}_N  \vvvert _{\Omega} \leq  \vvvert  \un{u}_N-\un{u}_D  \vvvert_{\Omega} + \sqrt{\sum_s\ecrc{\dep_N\s,\hat{\sig}_N\s}{\Omega\s}}
\end{equation}
\end{lem}
%
\begin{proof}
The proof of this lemma is based on the following result, proved in \cite{vohralik_posteriori_2007}:
 for $(\un{u},\depv) \in \KA(\Omega)\times\KA(\Omega)$ and $\widetilde{\un{u}} \in \broken$, 
\begin{equation}\label{eq:lemvohralik}
 \vvvert \un{u}-\widetilde{\un{u}} \vvvert_\Omega \leq \vvvert \depv-\widetilde{\un{u}} \vvvert_\Omega +
 \sum_s \int_{\Omega_s} \strain{\un{u}-\widetilde{\un{u}}}: \hooke :\strain{\frac{\un{u}-\depv}{\vvvert \un{u}-\depv \vvvert_\Omega}} d\Omega
 \end{equation}
%
We apply this result with $\un{u}=\un{u}_{ex}$ and $\widetilde{\un{u}}=(\un{u}_N\s)_s$, we note $\un{\varphi} = \frac{\un{u}_{ex}-\depv}{\vvvert \un{u}_{ex}-\depv\vvvert_\Omega}\in \KAo(\Omega)$, the second term of the expression is simplified by the introduction of $\hat{\sig}_N\s\in\SA(\Omega\s)$:
\begin{equation}
\begin{aligned}
% a(\un{u}_{ex}-\un{u}_N, \un{\varphi}) & = 
\sum_s \int_{\Omega_s} \strain{\un{u}_{ex}\s-\un{u}_N\s} :\hooke :\strain{\un{\varphi}\s} d\Omega &=
 \sum_s \int_{\Omega_s} (\sig_{ex}\s-\sig_N\s ) :\strain{\un{\varphi}\s} d\Omega \\
& = \sum_s \int_{\Omega_s} (\hat{\sig}_N\s-\sig_N\s ) :\strain{\un{\varphi}\s} d\Omega \\
& \leqslant \sum_s \lVert \hat{\sig}_N\s-\sig_N\s \rVert_{\hooke^{-1},\Omega\s} \vvvert \un{\varphi}\s\vvvert_{\Omega\s}\\
& \leqslant \sqrt{\sum_s \lVert \hat{\sig}_N\s-\sig_N\s \rVert_{\hooke^{-1},\Omega\s}^2}\\&\qquad\qquad\qquad\qquad\times \underbrace{\sqrt{\sum_s\vvvert \un{\varphi}\s\vvvert_{\Omega\s}^2}}_{=1}
\end{aligned}
\end{equation}
where we have used Cauchy-Schwarz inequality (two times). 
By definition  $\lVert \hat{\sig}_N\s-\sig_N\s \rVert_{\hooke^{-1},\Omega\s} = \ecr{\dep_N\s,\hat{\sig}_N\s}{\Omega\s}$. One just has to choose $\depv=\un{u}_D$ in the first term of  Equation~\eqref{eq:lemvohralik}.
\end{proof}

\begin{lem} Using the notation of algorithms~\ref{alg:bdd} or~\ref{alg:feti}, we have: 
\begin{equation}
\lVert \un{u}_N-\un{u}_D \rVert_{\hooke,\Omega}^2 = \res^T\bz
\end{equation}
in other words, the distance between $\un{u}_N$ and $\un{u}_D$ in the energy norm is the pre\-con\-di\-tio\-ner norm of the residual.
\end{lem}
\begin{proof}
Let us transform the expression of the first term using Stockes' theorem:
\begin{equation}
\begin{aligned}
\lVert \un{u}_N-\un{u}_D \rVert_{\hooke,\Omega}^2 &= \sum_s \int_{\Omega\s} \strain{\un{u}_D\s-\un{u}_N\s} : \hooke: \strain{\un{u}_D\s-\un{u}_N\s} d\Omega\\
&=   \sum_s \int_{\Gamma\s} \left( (\sig_D\s-\sig_N\s)\cdot \un{n}\s\right) \cdot \left(\un{u}_D\s-\un{u}_N\s\right)  d\Gamma\\& \qquad \  - \underbrace{ \sum_s \int_{\Omega\s} \diver(\sig_D\s-\sig_N\s)\cdot (\un{u}_D\s-\un{u}_N\s)d\Omega }_{=0}\\
&= 
 \sum_s \left(\lam_D\s-\lam_N\s\right)^T{\eft\s} \left(\efdep_D\s-\efdep_N\s\right)\\
 &=\sum_s\tlam\sT\tdep_b\s
\end{aligned}
\end{equation}
We now need to make particular cases depending on the algorithm. 
 In the  BDD case, we have:
\begin{equation}
\begin{aligned}
 \sum_s\tlam\sT\tdep_b\s = \sum_s (\tpa\sT \res)^T \tdep_b\s= \res^T \bz
\end{aligned}
\end{equation}
In the FETI case, we use the fact that $\res=\proj_2^T\res$:
\begin{equation}
\begin{aligned}
\sum_s\tlam\sT\tdep_b\s = \sum_s\tlam\sT \tda\sT \res= \sum_s\tlam\sT \tda\sT \proj_2^T\res = \res^T \bz
\end{aligned}
\end{equation}
\end{proof}



This leads to the resolution strategy of Algorithm~\ref{alg:ddstop}. The idea is to iterate until the algebraic error is negligible with respect to the estimation of the discretization error. 
\begin{algorithm2e}[th]\caption{DD solver with adapted stopping criterion}\label{alg:ddstop}
\DontPrintSemicolon
Set $\alpha>1$ and $\beta\geqslant 1$\;
Initialize, get $(\efdep_N\s,\lam_N\s,\res,\bz)$\;%
Estimate discretization error $e^2=\sum_s\ecrc{\dep_N\s,\hat{\sig}_N\s}{\Omega\s}$ \;
\While{$\sqrt{\res^T\bz}>e/\alpha$}{
\While{$\sqrt{\res^T\bz}>e/(\alpha \beta)$}{
Make Alg.~\ref{alg:bdd} or Alg.~\ref{alg:feti} iterations, get $(\efdep_N\s,\lam_N\s)$
}
Update error estimator $e^2=\sum_s\ecrc{\dep_N\s,\hat{\sig}_N\s}{\Omega\s}$ \;
}
\end{algorithm2e}
The objective being to have the norm of the residual $\alpha$ times smaller than the estimation of the discretization error ($\alpha=10$ is a typical value), the coefficient $\beta$ (typically 2) takes into account the small variation of the estimate $e$ of the discretization error along iterations.


%\subsection{New stopping criterion for the iterative solver}
%In this section, we propose a new upper bound that distincts the algebraic error from the discretization error. This result naturally leads us to define a new stopping criterion for the iterative solver. We stop the iterations when (algebraic~error~$\leq \frac{1}{10}$discretization~error). Therefore, we avoid useless and expensive iterations that cannont improve the global quality of the solution. Moreover, the map of the error provided by the estimator is helpful for a remesh procedure before a new computation.

